Recovering Dynamic 3D Sketches from Videos

Understanding 3D motion from videos presents inherent challenges due to the diverse types of movement, ranging from rigid and deformable objects to articulated structures. To overcome this, we propose Liv3Stroke, a novel approach for abstracting objects in motion with deformable 3D strokes. The detailed movements of an object may be represented by unstructured motion vectors or a set of motion primitives using a pre-defined articulation from a template model. Just as a free-hand sketch can intuitively visualize scenes or intentions with a sparse set of lines, we utilize a set of parametric 3D curves to capture a set of spatially smooth motion elements for general objects with unknown structures. We first extract noisy, 3D point cloud motion guidance from video frames using semantic features, and our approach deforms a set of curves to abstract essential motion features as a set of explicit 3D representations. Such abstraction enables an understanding of prominent components of motions while maintaining robustness to environmental factors. Our approach allows direct analysis of 3D object movements from video, tackling the uncertainty that typically occurs when translating real-world motion into recorded footage. The project page is accessible via: https://jaeah.me/liv3stroke_web

==> tables/4_quanti_sketch.tex <==
\begin{table*}[hbt]\setlength{\tabcolsep}{3pt}
\vspace{-4pt}
\setlength{\abovecaptionskip}{6.5pt}
\footnotesize
\centering 
\begin{tabular}{c c}

\begin{tabular}{lcccc} 
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{2}{c}{Strcutural alignment $\left(\uparrow\right)$} & \multicolumn{2}{c}{Motion prompt similarity $\left(\uparrow\right)$} \\
    & Novel views & Fixed views & Novel views & Fixed views \\
    \midrule 
    CLIPasso & $0.760 \pm 0.107$ & $0.740 \pm 0.127 $ & $0.659 \pm 0.007$ & $0.664 \pm 0.011$ \\
    Sketch Video Syn. & $0.663 \pm 0.115$ & $0.657 \pm 0.135$ & $0.654 \pm 0.011$ & $0.658 \pm 0.011$ \\
    % S-DyRF & $0.754 \pm 0.009$ & $0.965 \pm 0.003$ & $0.142 \pm 0.005$ & $0.142 \pm 0.005$ \\
    Sugg. Contours & $0.784 \pm 0.102$ & $0.750 \pm 0.119$ & $0.661 \pm 0.013$ & $0.656 \pm 0.016$ \\
    \midrule
    Liv3Stroke (Ours) & $0.693 \pm 0.096$ & $0.683 \pm 0.108$ & $0.656 \pm 0.006$ & $0.656 \pm 0.008$ \\
    \bottomrule \\
    \multicolumn{5}{c}{(a) Comparisons of structural alignment and motion prompt similarity.}
\end{tabular}

&

\begin{tabular}{lcccc}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{2}{c}{Novel views} & \multicolumn{2}{c}{Fixed views} \\
    & Motion & Structure & Motion & Structure \\
    \midrule 
    CLIPasso & $3.32$ & $3.08$ & $2.87$ & $2.70$ \\
    Sketch Video Syn. & $2.66$ & $2.64$ & $3.93$ & $3.77$ \\
    % S-DyRF & $0.754 \pm 0.009$ & $0.965 \pm 0.003$ & $0.142 \pm 0.005$ & $0.142 \pm 0.005$ \\
    Sugg. Contours & $4.26$ & $4.29$ & $3.82$ & $3.90$ \\
    \midrule
    Liv3Stroke (Ours) & $3.32$ & $3.08$ & $3.21$ & $2.94$ \\
    \bottomrule \\
    \multicolumn{5}{c}{(b) User study results of expression recognition.}
\end{tabular}

\end{tabular}
    \caption{Quantitative metrics on sketch video frames.
    \textbf{(a)} Structural alignment score with edge images of referenced frames and CLIP feature-based motion prompt similarity.
    \textbf{(b)} User study analysis of sketch expression recognition.
    It shows that our approach demonstrates consistent performance across different viewpoint scenarios.
}\label{tab:4_quant_sketch}

\vspace{-8pt}
\end{table*}
